UNIT: Backdoor Mitigation via Automated Neural Distribution Tightening

Deep neural networks (DNNs) have demonstrated effectiveness in various fields. However, DNNs are vulnerable to backdoor attacks, which inject a unique pattern, called trigger, into the input to cause misclassification to an attack-chosen target label. While existing works have proposed various methods to mitigate backdoor effects in poisoned models, they tend to be less effective against recent advanced attacks. In this paper, we introduce a novel post-training defense technique UNIT that can effectively eliminate backdoor effects for a variety of attacks. In specific, UNIT approximates a unique and tight activation distribution for each neuron in the model. It then proactively dispels substantially large activation values that exceed the approximated boundaries. Our experimental results demonstrate that UNIT outperforms 7 popular defense methods against 14 existing backdoor attacks, including 2 advanced attacks, using only 5\% of clean training data. UNIT is also cost efficient. The code is accessible at https://github.com/Megum1/UNIT.

==> Tables/ablation_degradation.tex <==
\begin{table}[t]
    \centering
    \footnotesize
    % \scriptsize
    % \renewcommand{\arraystretch}{1.2}
    \tabcolsep=5pt
    %\belowrulesep=0pt
    %\aboverulesep=0pt
    % \setlength{\belowcaptionskip}{5pt}
    \caption{Ablation study of different customized accuracy degradation.}
    \label{tab:ablation_degrade}
    \begin{tabular}{ccc}
         \toprule
         \textbf{Degradation} & \textbf{Accuracy} & \textbf{ASR} \\
         \midrule
         Origin & 94.73\% & 100.00\% \\
         \midrule
         0.01\% & 94.08\% & 4.01\% \\
         0.1\% & 93.89\% & 3.56\% \\
         1\% & 92.38\% & 2.17\% \\
         5\% & 88.36\% & 1.40\% \\
         10\% & 84.21\% & 1.12\% \\
         \bottomrule
    \end{tabular}
\end{table}


==> Tables/ablation_layers.tex <==
\begin{table*}[ht!]
    \centering
    \footnotesize
    % \scriptsize
    % \renewcommand{\arraystretch}{1.2}
    \tabcolsep=5.5pt
    %\belowrulesep=0pt
    %\aboverulesep=0pt
    % \setlength{\belowcaptionskip}{5pt}
    \caption{Ablation study of operation on different layers. Bad results (ASR $> 3\%$) are in bold.}
    \label{tab:ablation_layers}
    \begin{tabular}{cgcgcgcgcgc}
         \toprule
         \multirow{2}{*}{\textbf{Attacks}} & \multicolumn{2}{c}{\textbf{No Defense}} & \multicolumn{2}{c}{\textbf{Current Setting}} & \multicolumn{2}{c}{\textbf{Activation Rejection}} & \multicolumn{2}{c}{\textbf{First Layer}} & \multicolumn{2}{c}{\textbf{Last Layer}} \\
         \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11}
         ~ & \cellcolor{white}{Accuracy} & \cellcolor{white}{ASR} & \cellcolor{white}{Accuracy} & \cellcolor{white}{ASR} & \cellcolor{white}{Accuracy} & \cellcolor{white}{ASR} & \cellcolor{white}{Accuracy} & \cellcolor{white}{ASR} & \cellcolor{white}{Accuracy} & \cellcolor{white}{ASR} \\
         \midrule
         BadNets & 94.82\% & 100.00\% & 92.46\% & 0.78\% & 92.34\% & 1.56\% & 92.18\% & 0.54\% & 92.04\% & 0.74\% \\
         TrojNN & 94.73\% & 100.00\% & 92.44\% & 2.17\% & 92.50\% & \textbf{18.59\%} & 92.00\% & 1.04\% & 92.52\% & 1.96\% \\
         Dynamic & 95.08\% & 100.00\% & 92.77\% & 1.60\% & 92.43\% & 2.60\% & 92.76\% & 0.93\% & 92.70\% & 1.23\% \\
         InputAware & 91.15\% & 97.96\% & 89.96\% & 1.03\% & 90.52\% & 2.22\% & 90.05\% & 0.92\% & 90.13\% & 1.16\% \\
         SIG & 94.97\% & 99.80\% & 92.57\% & 1.78\% & 92.19\% & 2.54\% & 92.36\% & \textbf{7.57\%} & 92.30\% & 0.53\% \\
         Blend & 94.62\% & 100.00\% & 92.10\% & 1.18\% & 91.86\% & \textbf{9.66\%} & 92.23\% & 0.49\% & 91.93\% & 0.88\% \\
         WaNet & 94.36\% & 99.80\% & 91.33\% & \textbf{6.13\%} & 91.38\% & \textbf{5.54\%} & 91.81\% & \textbf{96.33\%} & 91.78\% & \textbf{51.08\%} \\
         Invisible & 94.55\% & 100.00\% & 91.94\% & 1.57\% & 91.65\% & 2.83\% & 92.03\% & \textbf{97.28\%} & 92.34\% & 2.08\% \\
         LIRA & 95.11\% & 100.00\% & 92.36\% & 0.59\% & 92.52\% & \textbf{6.31\%} & 92.35\% & 0.16\% & 92.22\% & 0.12\% \\
         \bottomrule
    \end{tabular}
\end{table*}


==> Tables/ablation_operation.tex <==
\begin{table*}[ht]
    \centering
    \footnotesize
    % \scriptsize
    % \renewcommand{\arraystretch}{1.2}
    \tabcolsep=4pt
    %\belowrulesep=0pt
    %\aboverulesep=0pt
    % \setlength{\belowcaptionskip}{5pt}
    \caption{Ablation study of different distribution statistics approximation methods. Best results are in bold.}
    \label{tab:ablation_operation}
    \begin{tabular}{cgcgcgcgcgc}
         \toprule
         \multirow{2}{*}{\textbf{Attacks}} & \multicolumn{2}{c}{\textbf{Original}} & \multicolumn{2}{c}{\textbf{Averaging $(N,)$}} & \multicolumn{2}{c}{\textbf{Averaging $(N, H, W)$}} & \multicolumn{2}{c}{\textbf{Averaging $(N, C, H, W)$}} & \multicolumn{2}{c}{\textbf{Rejecting}} \\
         \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11}
         ~ & \cellcolor{white}{Accuracy} & \cellcolor{white}{ASR} & \cellcolor{white}{Accuracy} & \cellcolor{white}{ASR} & \cellcolor{white}{Accuracy} & \cellcolor{white}{ASR} & \cellcolor{white}{Accuracy} & \cellcolor{white}{ASR} & \cellcolor{white}{Accuracy} & \cellcolor{white}{ASR} \\
         \midrule
         BadNets & 94.82\% & 100.00\% & 92.46\% & \textbf{0.78\%} & 92.65\% & 0.90\% & 92.74\% & \textbf{0.70\%} & 92.19\% & 0.89\% \\
         TrojNN & 94.73\% & 100.00\% & 92.44\% & \textbf{2.17\%} & 92.90\% & 3.03\% & 92.46\% & \textbf{1.96\%} & 92.57\% & 2.59\% \\
         Dynamic & 95.08\% & 100.00\% & 92.77\% & \textbf{1.60\%} & 92.66\% & 1.80\% & 92.59\% & \textbf{1.33\%} & 92.49\% & 1.78\% \\
         InputAware & 91.15\% & 97.96\% & 89.96\% & 1.03\% & 90.45\% & 1.16\% & 90.41\% & 5.21\% & 90.38\% & \textbf{0.99\%} \\
         SIG & 94.97\% & 99.80\% & 92.57\% & 1.78\% & 92.44\% & 2.39\% & 92.74\% & 56.44\% & 92.33\% & \textbf{0.70\%} \\
         Blend & 94.62\% & 100.00\% & 92.10\% & \textbf{1.18\%} & 92.13\% & 1.84\% & 92.49\% & 70.67\% & 91.74\% & 1.31\% \\
         WaNet & 94.36\% & 99.80\% & 92.34\% & 7.86\% & 91.61\% & 4.73\% & 91.92\% & 53.54\% & 91.65\% & \textbf{3.09\%} \\
         Invisible & 94.55\% & 100.00\% & 91.94\% & \textbf{1.57\%} & 92.07\% & 1.69\% & 92.36\% & 47.93\% & 92.01\% & 1.61\% \\
         LIRA & 95.11\% & 100.00\% & 92.36\% & \textbf{0.59\%} & 92.79\% & 0.60\% & 92.84\% & 63.17\% & 92.71\% & 0.71\% \\
         \bottomrule
    \end{tabular}
\end{table*}


==> Tables/ablation_steps.tex <==
\begin{table}[t]
    \centering
    \footnotesize
    % \scriptsize
    % \renewcommand{\arraystretch}{1.2}
    \tabcolsep=5pt
    %\belowrulesep=0pt
    %\aboverulesep=0pt
    % \setlength{\belowcaptionskip}{5pt}
    \caption{Ablation study of different approximation steps.}
    \label{tab:ablation_step}
    \begin{tabular}{ccccc}
         \toprule
         \textbf{Degradation} & \textbf{Accuracy} & \textbf{ASR} & \textbf{Theta} & \textbf{Time (s)} \\
         \midrule
         Origin & 94.73\% & 100.00\% & - & - \\
         \midrule
         2 & 94.01\% & 3.72\% & 5.000 & 2.82 \\
         5 & 91.27\% & 1.76\% & 3.125 & 3.17 \\
         10 & 92.38\% & 2.17\% & 3.535 & 4.56 \\
         20 & 92.43\% & 2.17\% & 3.543 & 6.64 \\
         50 & 92.43\% & 2.17\% & 3.543 & 13.46 \\
         \bottomrule
    \end{tabular}
\end{table}


==> Tables/baseline_0.1.tex <==
\begin{table*}[t]
    \centering
    \footnotesize
    % \scriptsize
    % \renewcommand{\arraystretch}{1.2}
    \tabcolsep=3pt
    %\belowrulesep=0pt
    %\aboverulesep=0pt
    % \setlength{\belowcaptionskip}{5pt}
    \caption{Effectiveness of \Tech{} compared with 4 backdoor removal methods against 9 backdoor attacks given 0.1\% of training data. The best results are in bold.}
    \label{tab:baseline_0.1}
    \begin{tabular}{cgcgcgcgcgcgc}
         \toprule
         \multirow{2}{*}{\textbf{Attacks}} & \multicolumn{2}{c}{\textbf{Original}} & \multicolumn{2}{c}{\textbf{Finetuning}} & \multicolumn{2}{c}{\textbf{Finepruning}} & \multicolumn{2}{c}{\textbf{NAD}} & \multicolumn{2}{c}{\textbf{ANP}} & \multicolumn{2}{c}{\textbf{\Tech{}}} \\
         \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13}
         ~ & \cellcolor{white}{Accuracy} & \cellcolor{white}{ASR} & \cellcolor{white}{Accuracy} & \cellcolor{white}{ASR} & \cellcolor{white}{Accuracy} & \cellcolor{white}{ASR} & \cellcolor{white}{Accuracy} & \cellcolor{white}{ASR} & \cellcolor{white}{Accuracy} & \cellcolor{white}{ASR} & \cellcolor{white}{Accuracy} & \cellcolor{white}{ASR} \\
         \midrule
         BadNets & 94.82\% & 100.00\% & 90.68\% & 2.24\% & 90.14\% & 7.62\% & 91.91\% & 2.08\% & 89.74\% & 1.43\% & \textbf{92.10\%} & \textbf{0.94\%} \\
         TrojNN & 94.73\% & 100.00\% & 91.28\% & 8.68\% & 90.03\% & 36.00\% & 91.51\% & 8.77\% & 91.69\% & 44.03\% & \textbf{92.14\%} & \textbf{3.00\%} \\
         Dynamic & 95.08\% & 100.00\% & 90.21\% & 4.40\% & 89.13\% & 10.28\% & 91.55\% & 3.07\% & \textbf{92.41\%} & \textbf{1.52\%} & 91.80\% & 1.86\% \\
         InputAware & 91.15\% & 97.96\% & 89.60\% & 96.18\% & 87.43\% & 99.77\% & 89.86\% & 95.91\% & 89.57\% & 14.93\% & \textbf{90.33\%} & \textbf{1.08\%} \\
         SIG & 94.97\% & 99.80\% & 91.86\% & 3.10\% & 78.94\% & 100.00\% & \textbf{92.09\%} & \textbf{1.87\%} & 85.85\% & 17.68\% & 91.94\% & 5.23\% \\
         Blend & 94.62\% & 100.00\% & 91.15\% & 3.53\% & 90.24\% & 47.36\% & 91.65\% & 2.04\% & 91.19\% & 13.87\% & \textbf{91.92\%} & \textbf{1.81\%} \\
         WaNet & 94.36\% & 99.80\% & 91.31\% & 23.68\% & 62.25\% & 99.98\% & 91.53\% & 18.29\% & 91.92\% & \textbf{0.77\%} & \textbf{92.63\%} & 5.31\% \\
         Invisible & 94.55\% & 100.00\% & 91.38\% & 2.96\% & 89.71\% & 6.51\% & 91.90\% & 2.51\% & 91.52\% & 62.99\% & \textbf{91.68\%} & \textbf{2.02\%} \\
         LIRA & 95.11\% & 100.00\% & 89.12\% & 15.09\% & 88.66\% & 17.69\% & 89.00\% & 8.85\% & 91.12\% & 74.71\% & \textbf{91.48\%} & \textbf{0.57\%} \\
         \midrule
         \textbf{Average} & 94.38\% & 99.73\% & 90.73\% & 17.76\% & 85.17\% & 47.25\% & 91.22\% & 15.93\% & 90.56\% & 25.77\% & \textbf{91.78\%} & \textbf{2.42\%} \\
         \bottomrule
    \end{tabular}
\end{table*}


==> Tables/baseline_10.tex <==
\begin{table*}[ht]
    \centering
    \footnotesize
    % \scriptsize
    % \renewcommand{\arraystretch}{1.2}
    \tabcolsep=3pt
    %\belowrulesep=0pt
    %\aboverulesep=0pt
    % \setlength{\belowcaptionskip}{5pt}
    \caption{Effectiveness of \Tech{} compared with 4 backdoor removal methods against 9 backdoor attacks given 10\% of training data. The best results are in bold.}
    \label{tab:baseline_10}
    \begin{tabular}{cgcgcgcgcgcgc}
         \toprule
         \multirow{2}{*}{\textbf{Attacks}} & \multicolumn{2}{c}{\textbf{Original}} & \multicolumn{2}{c}{\textbf{Finetuning}} & \multicolumn{2}{c}{\textbf{Finepruning}} & \multicolumn{2}{c}{\textbf{NAD}} & \multicolumn{2}{c}{\textbf{ANP}} & \multicolumn{2}{c}{\textbf{\Tech{}}} \\
         \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13}
         ~ & \cellcolor{white}{Accuracy} & \cellcolor{white}{ASR} & \cellcolor{white}{Accuracy} & \cellcolor{white}{ASR} & \cellcolor{white}{Accuracy} & \cellcolor{white}{ASR} & \cellcolor{white}{Accuracy} & \cellcolor{white}{ASR} & \cellcolor{white}{Accuracy} & \cellcolor{white}{ASR} & \cellcolor{white}{Accuracy} & \cellcolor{white}{ASR} \\
         \midrule
         BadNets & 94.82\% & 100.00\% & 91.54\% & 1.68\% & 91.13\% & 4.12\% & 92.15\% & 1.84\% & 92.21\% & 2.42\% & \textbf{92.45\%} & \textbf{0.89\%} \\
         TrojNN & 94.73\% & 100.00\% & 90.44\% & 13.34\% & 92.09\% & 7.99\% & 90.79\% & 16.56\% & 91.44\% & 38.29\% & \textbf{92.57\%} & \textbf{2.49\%} \\
         Dynamic & 95.08\% & 100.00\% & 89.81\% & 3.64\% & 90.94\% & 3.06\% & 90.15\% & 3.82\% & 90.99\% & 2.46\% & \textbf{92.49\%} & \textbf{1.74\%} \\
         InputAware & 91.15\% & 97.96\% & 91.93\% & 42.77\% & 91.33\% & 89.98\% & 91.97\% & 24.64\% & 89.46\% & 3.31\% & \textbf{90.58\%} & \textbf{0.99\%} \\
         SIG & 94.97\% & 99.80\% & 90.09\% & 0.81\% & 91.89\% & 3.67\% & 90.72\% & 0.99\% & 88.73\% & 34.53\% & \textbf{92.36\%} & \textbf{0.67\%} \\
         Blend & 94.62\% & 100.00\% & 91.22\% & 2.14\% & 91.78\% & \textbf{0.95\%} & 91.60\% & 1.78\% & 88.47\% & 10.34\% & \textbf{92.01\%} & 1.48\% \\
         WaNet & 94.36\% & 99.80\% & \textbf{92.81\%} & \textbf{0.52\%} & 91.77\% & 2.17\% & 92.64\% & 0.86\% & 90.44\% & 1.57\% & 91.64\% & 2.89\% \\
         Invisible & 94.55\% & 100.00\% & \textbf{93.08\%} & \textbf{1.14\%} & 91.13\% & 3.40\% & 93.09\% & 1.67\% & 92.03\% & 13.23\% & 92.26\% & 1.64\% \\
         LIRA & 95.11\% & 100.00\% & 90.43\% & 2.46\% & 91.24\% & 10.78\% & 90.59\% & 2.59\% & 89.51\% & 25.86\% & \textbf{92.57\%} & \textbf{0.64\%} \\
         \midrule
         \textbf{Average} & 94.38\% & 99.73\% & 91.26\% & 7.61\% & 91.48\% & 14.01\% & 91.52\% & 6.08\% & 90.36\% & 14.67\% & \textbf{92.10\%} & \textbf{1.49\%} \\
         \bottomrule
    \end{tabular}
\end{table*}


==> Tables/baseline_5.tex <==
\begin{table*}[ht]
    \centering
    \footnotesize
    % \scriptsize
    % \renewcommand{\arraystretch}{1.2}
    \tabcolsep=3pt
    %\belowrulesep=0pt
    %\aboverulesep=0pt
    % \setlength{\belowcaptionskip}{5pt}
    \caption{Effectiveness of \Tech{} compared with 4 backdoor removal methods against 9 backdoor attacks given 5\% of training data. The best results are in bold.}
    \label{tab:baseline_5}
    \begin{tabular}{cgcgcgcgcgcgc}
         \toprule
         \multirow{2}{*}{\textbf{Attacks}} & \multicolumn{2}{c}{\textbf{Original}} & \multicolumn{2}{c}{\textbf{Finetuning}} & \multicolumn{2}{c}{\textbf{Finepruning}} & \multicolumn{2}{c}{\textbf{NAD}} & \multicolumn{2}{c}{\textbf{ANP}} & \multicolumn{2}{c}{\textbf{\Tech{}}} \\
         \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13}
         ~ & \cellcolor{white}{Accuracy} & \cellcolor{white}{ASR} & \cellcolor{white}{Accuracy} & \cellcolor{white}{ASR} & \cellcolor{white}{Accuracy} & \cellcolor{white}{ASR} & \cellcolor{white}{Accuracy} & \cellcolor{white}{ASR} & \cellcolor{white}{Accuracy} & \cellcolor{white}{ASR} & \cellcolor{white}{Accuracy} & \cellcolor{white}{ASR} \\
         \midrule
         BadNets & 94.82\% & 100.00\% & 92.01\% & 4.29\% & 85.68\% & 3.52\% & 92.41\% & 4.79\% & 91.35\% & 3.26\% & \textbf{92.48\%} & \textbf{0.78\%} \\
         TrojNN & 94.73\% & 100.00\% & 91.22\% & 14.85\% & 90.76\% & 31.14\% & 91.52\% & 22.30\% & 92.37\% & 58.88\% & \textbf{92.38\%} & \textbf{2.17\%} \\
         Dynamic & 95.08\% & 100.00\% & 89.11\% & 2.36\% & 84.93\% & 3.23\% & 89.26\% & 2.34\% & 91.99\% & 3.09\% & \textbf{92.77\%} & \textbf{1.54\%} \\
         InputAware & 91.15\% & 97.96\% & 88.44\% & 2.92\% & 89.71\% & 82.20\% & 88.51\% & 2.67\% & 89.05\% & 5.49\% & \textbf{89.93\%} & \textbf{1.03\%} \\
         SIG & 94.97\% & 99.80\% & 91.29\% & 16.12\% & 90.88\% & \textbf{1.03\%} & 91.69\% & 10.46\% & 90.80\% & 36.79\% & \textbf{92.48\%} & 1.74\% \\
         Blend & 94.62\% & 100.00\% & 91.48\% & 1.72\% & 91.47\% & 2.01\% & 91.62\% & 3.32\% & 91.04\% & 16.79\% & \textbf{91.99\%} & \textbf{1.18\%} \\
         WaNet & 94.36\% & 99.80\% & 92.24\% & 1.28\% & 91.48\% & 1.48\% & \textbf{92.36\%} & 1.91\% & 91.99\% & \textbf{0.61\%} & 91.33\% & 6.13\% \\
         Invisible & 94.55\% & 100.00\% & 92.16\% & 1.67\% & 90.79\% & 2.11\% & \textbf{92.45\%} & 2.43\% & 92.42\% & 2.98\% & 91.84\% & \textbf{1.57\%} \\
         LIRA & 95.11\% & 100.00\% & 91.37\% & 2.02\% & 89.58\% & 14.76\% & 91.64\% & 2.06\% & 91.98\% & 47.91\% & \textbf{92.29\%} & \textbf{0.58\%} \\
         \midrule
         \textbf{Average} & 94.38\% & 99.73\% & 91.04\% & 5.25\% & 89.48\% & 15.72\% & 91.27\% & 5.81\% & 91.44\% & 19.53\% & \textbf{91.94\%} & \textbf{1.86\%} \\
         \bottomrule
    \end{tabular}
\end{table*}


==> Tables/robust_diff_rates.tex <==
\begin{table}[t]
    \centering
    \footnotesize
    % \scriptsize
    % \renewcommand{\arraystretch}{1.2}
    \tabcolsep=3pt
    %\belowrulesep=0pt
    %\aboverulesep=0pt
    % \setlength{\belowcaptionskip}{5pt}
    \caption{Robustness against different poisoning rates.}
    \label{tab:robust_diff_rates}
    \begin{tabular}{cgcgc}
         \toprule
         \multirow{2}{*}{\textbf{Poisoning Rate}} & \multicolumn{2}{c}{\textbf{Original}} & \multicolumn{2}{c}{\textbf{\Tech{}}} \\
         \cmidrule(lr){2-3} \cmidrule(lr){4-5}
         ~ & \cellcolor{white}{Accuracy} & ASR & \cellcolor{white}{Accuracy} & ASR \\
         \midrule
         1\% & 94.62\% & 100.00\% & 92.44\% & 1.00\% \\
         5\% & 94.67\% & 100.00\% & 92.27\% & 1.22\% \\
         10\% & 94.66\% & 100.00\% & 92.59\% & 1.02\% \\
         25\% & 95.00\% & 100.00\% & 92.38\% & 1.24\% \\
         50\% & 94.88\% & 100.00\% & 92.42\% & 1.29\% \\
         \bottomrule
    \end{tabular}
\end{table}


==> Tables/robust_diff_targets.tex <==
\begin{table}[t]
    \centering
    \footnotesize
    % \scriptsize
    % \renewcommand{\arraystretch}{1.2}
    \tabcolsep=3pt
    %\belowrulesep=0pt
    %\aboverulesep=0pt
    % \setlength{\belowcaptionskip}{5pt}
    \caption{Robustness against different attack target labels.}
    \label{tab:robust_diff_targets}
    \begin{tabular}{cgcgc}
         \toprule
         \multirow{2}{*}{\textbf{Target Label}} & \multicolumn{2}{c}{\textbf{Original}} & \multicolumn{2}{c}{\textbf{\Tech{}}} \\
         \cmidrule(lr){2-3} \cmidrule(lr){4-5}
         ~ & \cellcolor{white}{Accuracy} & ASR & \cellcolor{white}{Accuracy} & ASR \\
         \midrule
         1 & 94.85\% & 100.00\% & 92.59\% & 0.30\% \\
         3 & 94.93\% & 100.00\% & 92.44\% & 2.47\% \\
         5 & 94.56\% & 100.00\% & 92.68\% & 0.87\% \\
         7 & 94.78\% & 100.00\% & 92.48\% & 0.37\% \\
         9 & 94.87\% & 100.00\% & 92.59\% & 0.53\% \\
         \bottomrule
    \end{tabular}
\end{table}


==> Tables/theta_diff_models.tex <==
\begin{table}[t]
    \centering
    % \footnotesize
    \scriptsize
    % \tiny
    \tabcolsep=1pt
    \caption{Impact of $\eta$ on different datasets/networks. Best results are in bold when accuracy degradation is within 3\%.}
    \label{tab:theta_diff_models}
    \begin{tabular}{llcgcgcg}
         \toprule
         \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Network}} & \multicolumn{2}{c}{\textbf{$\eta=3.5$}} & \multicolumn{2}{c}{\textbf{$\eta=4.0$}} & \multicolumn{2}{c}{\textbf{$\eta=4.5$}} \\
         \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}
         ~ & ~ & \cellcolor{white}{Acc. Deg.} & \cellcolor{white}{ASR} & \cellcolor{white}{Acc. Deg.} & \cellcolor{white}{ASR} & \cellcolor{white}{Acc. Deg.} & \cellcolor{white}{ASR} \\
         \midrule
         CIFAR-10 & VGG11 & -3.30\% & 4.07\% & \textbf{-1.92\%} & \textbf{5.60\%} & -1.23\% & 7.50\% \\
         CIFAR-10 & ResNet18 & \textbf{-2.40\%} & \textbf{2.13\%} & -1.48\% & 2.62\% & -1.04\% & 3.06\% \\
         CIFAR-100 & Densenet & -6.55\% & 0.08\% & -3.92\% & 0.16\% & \textbf{-2.48\%} & \textbf{0.27\%} \\
         CIFAR-100 & Mobilenet & -4.22\% & 0.00\% & \textbf{-2.25\%} & \textbf{0.01\%} & -1.19\% & 0.03\% \\
         STL-10 & WideResNet & \textbf{-2.20\%} & \textbf{8.65\%} & -0.96\% & 14.50\% & -0.45\% & 24.22\% \\
         GTSRB & PRN34 & \textbf{-0.06\%} & \textbf{2.32\%} & -0.08\% & 2.59\% & -0.05\% & 2.89\% \\
         \bottomrule
    \end{tabular}
\end{table}


==> Tables/time_cost.tex <==
\begin{table}[t]
    \centering
    \footnotesize
    % \scriptsize
    % \renewcommand{\arraystretch}{1.2}
    \tabcolsep=2pt
    %\belowrulesep=0pt
    %\aboverulesep=0pt
    % \setlength{\belowcaptionskip}{5pt}
    \caption{\sy{Make it as a figure} Efficiency of \Tech{} compared with 4 backdoor removal methods against 9 backdoor attacks given 5\% of training data. The best results are in bold.}
    \label{tab:time_cost}
    \begin{tabular}{ccccccc}
         \toprule
         \textbf{Attack} & \textbf{Finetuning} & \textbf{Finepruning} & \textbf{NAD} & \textbf{ANP} & \textbf{\Tech{}} \\
         \midrule
         BadNets & 6.29 & 6.26 & 10.85 & 16.04 & 4.56 \\
         TrojNN & 6.31 & 6.36 & 10.86 & 16.43 & 4.54 \\
         Dynamic & 6.39 & 6.22 & 10.53 & 16.03 & 4.55 \\
         InputAware & 6.44 & 6.39 & 10.78 & 16.18 & 4.49 \\
         SIG & 6.41 & 6.32 & 10.71 & 16.71 & 4.52 \\
         Blend & 6.26 & 6.16 & 10.56 & 16.21 & 4.63 \\
         WaNet & 6.26 & 6.39 & 10.8 & 16.15 & 4.58 \\
         Invisible & 6.33 & 6.2 & 10.6 & 16.75 & 4.59 \\
         LIRA & 6.38 & 6.22 & 10.53 & 15.85 & 4.65 \\
         \bottomrule
    \end{tabular}
\end{table}

